Holomorphic Curves in Moduli Spaces Are Quasi-Isometrically Immersed

A holomorphic curve in moduli spaces is the image of a non-constant holomorphic map from a hyperbolic surface $B$ of type $(g,n)$ to the moduli space $\mathcal{M}_h$ of closed Riemann surfaces of genus $h$. We show that, when all peripheral monodromies are of infinite order, the holomorphic map is a quasi-isometric immersion with parameters depending only on $g$, $n$, $h$ and the systole of $B$. When peripheral monodromies also satisfy an additional condition, we find a lift quasi-isometrically embedding a fundamental polygon of the hyperbolic surface $B$ into the Teichm\"uller space. We further improve the Parshin-Arakelov finiteness theorem, by proving that there are only finitely many monodromy homomorphisms induced by holomorphic curves of type $(g,n)$ in $\mathcal{M}_h$ where systole is bounded away from $0$, up to equivalence.

==> Preliminary/BersMaskit.tex <==
\subsection{Bers-Maskit slice}
\label{subsection::Bers}

The following proposition is the most technical step in our study on the Parshin-Arakelov finiteness,
which first appeared in \cite{ImayoshiShiga1988} as part of the proof of the Parshin-Arakelov finiteness.
Shiga later formally formulated this result in \cite{Shiga1997}.
McMullen has also introduced a weak version when $n=0$ using the maximum principle for subharmonic functions (see Irreducibility in the proof of Theorem 3.1 in \cite{McMullen2000}).

\begin{proposition}
\label{proposition::no_disjoint_simple_loops_preserved}
Let $B$ be an oriented hyperbolic surface of type $(g,n)$ and 
$F:B\rightarrow \mathcal{M}_h$ be a non-constant holomorphic map.
Suppose that $F_*:\pi_1(B,t)\rightarrow \Mod_h$ is a monodromy homomorphism induced by $F$ with $t\in B$.
Then there does not exist a set of non-homotopic disjoint simple closed curves $\{\alpha_1,\ldots,\alpha_{h'}\}$ on $\Sigma_h$
such that the set of homotopy classes $\{[\alpha_1],\ldots,[\alpha_{h'}]\}$ is preserved by $F_*(g)$ for each $g\in\pi_1(B,t)$.
\end{proposition}

This subsection revisits Kleinian groups and the analytic structure of Teichm\"uller spaces that were first introduced by Bers (\cite{Bers1970}) and Maskit (\cite{Maskit1970}).
We include a proof of Proposition \ref{proposition::no_disjoint_simple_loops_preserved} at the end.\\

%%%%%%

\textbf{Projective linear group.}
By convention, we use $\hat{\C}$ to denote the Riemann sphere and the upper (resp. lower) half plane is expressed by $\mathcal{U}$ (resp. $\mathcal{L}$) $\subset \C\subset \hat{\C}$, where $\Hyperbolic^2=\mathcal{U}$.
The matrix group $\PSL(2,\mathbb{C})$ acts on $\hat{\mathbb{C}}$ via M\"obius transformations.
An element $1\neq g\in\PSL(2,\C)$ is called \emph{parabolic} if $\text{tr}^2(g)=4$,
\emph{elliptic} if $\text{tr}^2(g)\in (0,4)\subset \mathbb{R}$ and
\emph{loxodromic} in all other cases.
A loxodromic or elliptic element $g\in \PSL(2,\C)$ is diagonalizable and conjugate to a transformations
$z\rightarrow \lambda_{g} z$
with $|\lambda_{g}|\ge 1$, where $\lambda_{g}$ is called the \emph{multiplier}.

The matrix group $\PSL(2,\R)$ is regarded as the largest subgroup of $\PSL(2,\C)$ that fixes the upper half plane $\mathcal{U}$.
The natural embedding takes hyperbolic, parabolic and elliptic elements
into loxodromic, parabolic and elliptic elements, respectively.
Therefore, the multiplier $\lambda_g$ of any 2hyperbolic element $g\in\PSL(2,\R)$ is real and positive such that the translation dlength of $g$ is exactly $\log{\lambda_g}$.
We always suppose that a Fuchsian group $\Gamma\le \PSL(2,\R)$ is finitely generated and of the first type.

Let $G$ be an arbitrary subgroup of $\PSL(2,\C)$. The \emph{limit set} $\Lambda(G)$ is the closure of the set of fixed points of parabolic and loxodromic elements of G. Besides, $\Lambda(G)$ is also the set of accumulation points of orbits $Gz=\{g(z)\mid g\in G\}$.\\

%%%%%%

\textbf{Kleinian group.}
A \emph{Kleinian group} $G$ is a discrete subgroup of $\PSL(2,\C)$ that acts discontinuously on some open subset of $\hat{\C}$.
We always suppose that a Kleinian group is finitely generated and \emph{non-elementary}, i.e. $\Lambda(G)$ has more than two points.
The subset $\Omega(G)=\hat{\C}\setminus \Lambda(G)$ is the largest open set on which $G$ acts discontinuously.
If there exists a simply-connected component $\Delta$ of $\Omega(G)$ that is invariant under $G$, then $G$ is called a \emph{$B$-group}.
A $B$-group for which $\Omega(G)=\Delta$ is simply connected is called a \emph{totally degenerate group}.

If $G$ is a $B$-group with some invariant simply-connected component $\Delta\subset \Omega(G)\subset \hat{\C}$,
then there exists a conformal bijection 
$w_{\Delta}:\mathcal{U}\rightarrow\Delta$ (or $w_{\Delta}:\mathcal{L}\rightarrow\Delta$)
so that 
$w^{-1}Gw\le \PSL(2,\R)\le \PSL(2,\C)$
is a Fuchsian group isomorphic to $G$, called the \emph{Fuchsian equivalent} of $G$.
The isomorphism $G\ni g\mapsto w^{-1}gw\in w^{-1}Gw$ is denoted by $\chi_{w_{\Delta}}$.
If $\chi_{w_{\Delta}}$
sends a parabolic element $g\in G$ to a hyperbolic element,
then $g$ is called \emph{accidental parabolic} 
under the group isomorphism.

\begin{lemma}
\label{lemma::totally_degenerate}
Let $G$ be a $B$-group with
exactly one invariant simply-connected component $\Delta$ of $\hat{\C}\setminus\Lambda(G)$.
If there is no accidental parabolic element under $\chi_{w_{\Delta}}$, then $G$ is totally degenerate.
\end{lemma}

\begin{proof}
    See the corollary to Proposition 7 in \cite{Bers1970} or Theorem 4 in \cite{Maskit1970}.
\end{proof}

%%%%%%

\textbf{Quasi-Fuchsian group.}
A \emph{quasi-Fuchsian} group $G\le \PSL(2,\C)$ is a Kleinian group such that there exists an invariant (directed) Jordan curve $C\subset \hat{\C}$,
which implies a pair of Fuchsian groups $(G^{\mathcal{L}}$, $G^{\mathcal{U}})$.
Suppose that $\Delta^{\mathcal{L}}$, $\Delta^{\mathcal{U}}$ are connected components of $\hat{\C}\setminus C$
and
consider the corresponding conformal bijections $w^{\mathcal{L}}:\mathcal{L}\rightarrow \Delta^{\mathcal{L}}$, $w^{\mathcal{U}}:\mathcal{U}\rightarrow \Delta^{\mathcal{U}}$.
Therefore, $(G^{\mathcal{L}}$, $G^{\mathcal{U}})=(\chi_{w^{\mathcal{L}}}(\mathcal{U}),\chi_{w^{\mathcal{U}}}(\mathcal{U}))$.\\

%%%%%%

\textbf{Bounded quadratic differentials.}
Let $\Gamma\le \PSL(2,\R)$ be a Fuchsian group.
In \cite{Bers1970},
Bers introduced the finite dimensional complex Banach space $B_2(\mathcal{L},\Gamma)$ of \emph{bounded quadratic differentials} for $\Gamma$ in the lower half plane $\mathcal{L}$,
i.e. holomorphic functions $\phi:\mathcal{L}\rightarrow \mathbb{C}$ such that
$|(\Image(z)^2\phi(z)|$ is bounded
and
$\phi(g(z))g'(z)^2=\phi(z)$ for each $g\in \Gamma$.

For each $\phi \in B_2(\mathcal{L},\Gamma)$,
there exists a conformal Schwarzian antiderivative of $\phi$, denoted by $w_{\phi}:\mathcal{L}\rightarrow \hat{\C}$.
Therefore, the following group homomorphism sends $\Gamma$ to a Kleinian group $\Gamma_{\phi}$.
%\footnote{In \cite{Bers1970}, the group homomorphism is denoted by $\chi_{\phi}$ whose image $\Gamma_{\phi}$ is called the monodromy group of $\phi$. To avoid ambiguity, we do not address them like so.}
\begin{equation*}
g\ni\gamma \mapsto
\Xi_{\phi}(g)\coloneqq
w_{\phi}g w_{\phi}^{-1}\in
w_{\phi}\Gamma w_{\phi}^{-1}
\eqqcolon \Gamma_{\phi}
\le \PSL(2,\C).
\end{equation*}

\begin{lemma}[Lemma 2 in \cite{Bers1970}]
\label{lemma::trace_map_holomorphic_on_B2}
Let $\Gamma\le \PSL(2,\R)$ be a Fuchsian group.
Then, for any $g\in\Gamma$, the function
$\phi\mapsto \trace^2(\Xi_{\phi}(g))$
is holomorphic defined in $B_2(\mathcal{L},\Gamma)$.
\end{lemma}

We define $\Teich(\Gamma)\subset B_2(\mathcal{L},\Gamma)$, now known as the Bers-Maskit slice, as the set of $\phi\in B_2(\mathcal{L},\Gamma)$
such that $w_{\phi}$ admits a quasiconformal extension, denoted by $\hat{w}_{\phi}$, to all of $\hat{\C}$.
For any $\phi\in\Teich(\Gamma)$, the Kleinian group
$\Gamma_{\phi}$
is a quasi-Fuchsian group with invariant Jordan curve $w_{\phi}(\partial \mathcal{U})$, which implies a pair of Fuchsian groups 
$(\Gamma_{\phi}^{\mathcal{L}},\Gamma_{\phi}^{\mathcal{U}})$
but one is exactly $\Gamma$.
By convention,
we suppose that $\Gamma=\Gamma_{\phi}^{\mathcal{L}}$ and call $\Gamma_{\phi}^{\mathcal{U}}$ the \emph{upper equivalent} of $\Gamma_{\phi}$.
There exists a natural isomorphism between Fuchsian groups $\Gamma=\Gamma_{\phi}^{\mathcal{L}}$ and $\Gamma_{\phi}^{\mathcal{U}}$, denoted by $\hat{\Xi}_{\phi}$,
which further induces a quasiconformal map of $\mathcal{U}$.

\begin{lemma}
\label{lemma::Bers-Maskit slice}
Given a Fuchsian group $\Gamma$, we have the following statements.

\begin{enumerate}
[(i),topsep=0pt,itemsep=-1ex,partopsep=1ex,parsep=1ex]
\item The Bers-Maskit slice $\Teich(\Gamma)$ is bounded in $B_2(\mathcal{L},\Gamma)$.

\item For any $\phi\in \overline{\Teich(\Gamma)}$,
then $\Xi_{\gamma}:\Gamma\rightarrow \Gamma_{\phi}$ is an isomorphism to a Kleinian group.

\item For any $\phi\in \partial\Teich(\Gamma_0)$,
then $\Gamma_{\phi}$ is a $B$-group that contains precisely one invariant component $\Delta$, which is called a \emph{boundary group}.
\end{enumerate}
\end{lemma}

\begin{proof}
Assertion (\RNum{1}) comes from
the famous Nehari–Kraus's theorem.
Assertion (\RNum{2}) comes from Theorem 5 in \cite{Bers1970}.
Assertion (\RNum{3}) comes from Theorem 8 in \cite{Bers1970} where the invariant component $\Delta$ is hence simply-connected and $\chi_{w}(\Gamma_{\phi})$ is a Fuchsian equivalent of the boundary group, for some conformal bijection $w:\mathcal{U}\rightarrow \Delta$.
\end{proof}

%%%%%%

\textbf{Bers embedding of Teichm\"uller space.}
Suppose that the base point $[(X_0,f_{X_0})]\in \Teich_h$ has the hyperbolic representative $(X_0,f_{X_0})$ where $X_0$ is induced by a Fuchsian group $\Gamma_0\le \PSL(2,\R)$.
Teichm\"uller space $\Teich_h$ is interpreted as the space of equaivalent classes of quasiconformal maps of $\mathcal{U}=\Hyperbolic^2$ compatible with $\Gamma_0$, where two quasiconformal maps are equivalent if they coincide on the boundary up to pre-composition by M\"obius transformations.

Given a quasiconformal map $w:\mathcal{U}\rightarrow\mathcal{U}$,
Teichm\"uller space $\Teich_h$ can be identified with $\Teich(\Gamma_0)$
by taking the Schwarzian derivative $\phi$ of a natural extension $\hat{w}$ of $w$.
In fact, the quasiconformal map induced by $\hat{\Xi}_{\phi}$ is equivalent to $w$.
The analytic structure on $\Teich_h=\Teich(\Gamma_0)$ comes from the Banach space $B_2(\mathcal{L},\Gamma_0)$ and it is a bounded domain of a finite dimensional complex Banach space.

\begin{lemma}[Abikoff's lemma]
\label{lemma::abikoff}
Take $\phi\in\partial\Teich(\Gamma_0)$ such that
the boundary group $\Gamma_{\phi}$ is totally degenerate and
let $g\in\Gamma_{\phi}$ be a loxodromic element.
If there exist a sequence $\{\phi_n\}$ in $\Teich(\Gamma_0)$ that converges to $\phi$ as $n\rightarrow\infty$
and some hyperbolic $g_0\in \Gamma_0$ such that
$g_n\coloneqq \Xi_{\phi_n}(g_0) \in \Gamma_{\phi_n}\le \PSL(2,\C)$ 
converges to $g$ as $n\rightarrow\infty$, then
$L_{f_{X_0}^{-1}(\gamma_0)}(\phi_n)$
is unbounded, where $\gamma_0\subset X_0$ is an arbitrary closed curve corresponding to $g_0$
\end{lemma}

\begin{proof}
See Theorem 2 in \cite{Abikoff1976twotheorems}
and use the fact that
$L_{f_{X_0}^{-1}(\gamma_0)}(\phi_n)=\lambda_{\hat{\Xi}_{\phi_n}(g_0)}$.
\end{proof}

% bd group is discrete -> no elliptic element
% hyperbolic in Fuchsian -> loxidromic
% multiplier of loxidromic

%%%%%%

Now we prove Proposition \ref{proposition::no_disjoint_simple_loops_preserved}.

\begin{proof}[Proof of Proposition \ref{proposition::no_disjoint_simple_loops_preserved}]

Consider the non-constant holomorphic map $F:B\rightarrow \mathcal{M}_h$.
Let $\Delta\subset \C$ be the unit disc
and suppose that 
$\iota:\Delta\rightarrow B$ 
is a universal covering
whose cover transformation group is $\pi_1(B,t)$.
Therefore, $F$ induces the non-constant holomorphic map of the unit disc $\Delta$ to $\Teich_h$, denoted by $\widetilde{F}:\Delta \rightarrow \Teich_h$.

For each $g\in \pi_1(B,t)$ and $\alpha_i$, we have
\begin{equation*}
L_{\alpha_i}(\widetilde{F}(g(0)))
=
L_{F_*(g)(\alpha_i)}(\widetilde{F}(0))
\le
\max\{L_{\alpha_j}(\widetilde{F}(0))  \mid j=1,\ldots,h'\}.
\end{equation*}

Since $\widetilde{F}(\Delta)\subset\Teich_h= \Teich(\Gamma_0)\subset B_2(\mathcal{L},\Gamma_0)$ is bounded,
Fatou's theorem concerning holomorphic maps on the unit disc
states that for almost all $\zeta\in\partial \Delta$,
the holomorphic map $\widetilde{F}$ converges to some point
$q\in\overline{\Teich(\Gamma_0)}$ non-tangentially.
Since the cover transformation group $\pi_1(B,t)$ is of divergence type, there exists a sequence of transformations 
$g_{\zeta,j}\in \pi_1(B,t)$
such that $g_{\zeta,j}(z_0)$ converges to $\zeta$ non-tangentially and $\widetilde{F}(g_{\zeta,j}(z_0))$ converges to $q$ as $j\rightarrow\infty$,
for every $z_0\in\Delta$ (see Theorem \URNum{11} 20 in \cite{Tsuji1975}).

We claim that the image limit $q\in \partial\Teich(\Gamma_0)$.
Indeed, the monodromy $F_*(g_{\zeta,j})\in\Mod_h$ along $g_{\zeta,j}$ is a transformation on $\Teich_h=\Teich(\Gamma_0)$, which is isometric and holomorphic.
These transformations converge to a holomorphic map $A:\Teich_h\rightarrow\overline{\Teich_h}$.
Since $z_0$ is arbitrary,
if $q\in\Teich_h$ then $A$, as the limit of a sequence of isometries, cannot be constant, which is a contradiction.

By Lemma \ref{lemma::totally_degenerate} and Lemma \ref{lemma::Bers-Maskit slice} - (\RNum{3}),
if a boundary group $\Gamma_q$, for $q\in\partial \Teich(\Gamma_0)$, has no accidenal parabolic element, then $\Gamma_q$ is totally degenerate.
However, by Lemma \ref{lemma::trace_map_holomorphic_on_B2} and Lemma \ref{lemma::Bers-Maskit slice} - (\RNum{1}),
the bounded holomorphic map
\begin{equation*}
\Delta\ni z
\mapsto
\trace^2(\Xi_{\widetilde{F}(z)}(g))
\end{equation*}
cannot have non-tangential limits that is equal to $4$ almost everywhere on $\partial \Teich(\Gamma_0)$,
for each hyperbolic transformation $g\in \Gamma_0$.
Besides, $\Gamma_0$ is finitely generated and therefore countable.
Hence, for almost all possible non-tangential image limits $q\in \partial \Teich(\Gamma_0)$ of $\widetilde{F}$,
boundary groups $\Gamma_q$ are totally degenerate.

Let $\zeta\in \partial\Delta$ be a boundary point and $g_{\zeta,j}\in \pi_1(B,t)$ be a sequence of transformations such that
$g_{\zeta,j}(0)\eqqcolon z_j\in \Delta$ converges to $\zeta\in\partial\Delta$ non-tangentially,
$\widetilde{F}(z_j)$ converges to $q \in\partial \Teich(\Gamma_0)$ as $j\rightarrow\infty$,
the boundary group $\Gamma_q\le \PSL(2,\C)$ is totally degenerate and has no accidental parabolic element under $\Xi_q^{-1}:\Gamma_q\rightarrow \Gamma_0$.
Let $g_0\in\Gamma_0$ be hyperbolic and corresponding to $f_{X_0}(\alpha_i)\subset X_0$.
By Lemma \ref{lemma::Bers-Maskit slice} - (\RNum{2}), transformations $\Xi_{\widetilde{F}(z_j)}(g_0)$ must converge to a loxodromic element $\Xi_q(g_0)$.
By Lemma \ref{lemma::abikoff}, we get
\begin{equation*}
L_{\alpha_i}(\widetilde{F}(z_j))
\rightarrow\infty
\text{ as }
j\rightarrow\infty,
\end{equation*}
a contradiction.
\end{proof}
